MPBench: A Comprehensive Multimodal Reasoning Benchmark for Process Errors Identification

Reasoning is an essential capacity for large language models (LLMs) to address complex tasks, where the identification of process errors is vital for improving this ability. Recently, process-level reward models (PRMs) were proposed to provide step-wise rewards that facilitate reinforcement learning and data production during training and guide LLMs toward correct steps during inference, thereby improving reasoning accuracy. However, existing benchmarks of PRMs are text-based and focus on error detection, neglecting other scenarios like reasoning search. To address this gap, we introduce MPBench, a comprehensive, multi-task, multimodal benchmark designed to systematically assess the effectiveness of PRMs in diverse scenarios. MPBench employs three evaluation paradigms, each targeting a specific role of PRMs in the reasoning process: (1) Step Correctness, which assesses the correctness of each intermediate reasoning step; (2) Answer Aggregation, which aggregates multiple solutions and selects the best one; and (3) Reasoning Process Search, which guides the search for optimal reasoning steps during inference. Through these paradigms, MPBench makes comprehensive evaluations and provides insights into the development of multimodal PRMs.

==> tables/abla.tex <==
\begin{table}[!ht]\centering
  \footnotesize
  \renewcommand{\arraystretch}{1.0}
  \renewcommand{\tabcolsep}{1.1mm}
\resizebox{0.48\textwidth}{!}{\begin{tabular}{l|c|c|c|ccc}\toprule
\multirow{2}{*}{ Method }  & { VQAv2} & { \nlvr} & { VE} & \multicolumn{3}{c}{ Flickr30k} \\
 & { Test-Dev} & { Test-P} & { Test} & { R@1} & { R@5} & { R@10} \\\cmidrule{1-7}

Tag-Retrieval &73.3 & 74.6 & 78.2 &67.4 & 90.2 & 95.1\\
IST &73.5&76.6&78.5&74.5  & 92.0 & 96.2 \\
TSI &73.6&77.3&78.9& 77.7 & 93.1 & 96.8 \\
IST+TSI & \textbf{73.8} & \textbf{77.6} & \textbf{79.4}  & \textbf{80.6} & \textbf{95.3} & \textbf{98.4} \\
\bottomrule
\end{tabular}}
\caption{Ablation studies on components of RGSC .}
\label{tab:abla}
\end{table}

==> tables/fewshot.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{p{\textwidth}}
\toprule
Question: \{question\}\\
Answer: \{response\}\\
Review your previous answer and find problems with your answer.\\
Finally, conclude with either '[[correct]]' if the above answer is correct or '[[wrong]]' if it is incorrect.\\
Verdict: \\
\bottomrule
\end{tabular}
\caption{Zero-shot Answer Only Prompt for Critique}
\end{table*}
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{\textwidth}}
\toprule
Question: \{question\} \\
Answer: \{response\} \\
Review your previous answer and find problems with your answer. \\
Provide your analysis and verdict in JSON format as follows: \{"analysis": "your analysis", "verdict": "correct or wrong"\}. \\
Analysis and verdict:  \\
\bottomrule
\end{tabular}
}
\caption{Zero-shot Chain of Thought Prompt for Critique}
\end{table*}

\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{\textwidth}}
\toprule
Review the above answer and determine whether it’s correct. If wrong, find the problems with it.\\
Finally, conclude with either '[[correct]]' if the above answer is correct or '[[wrong]]' if it is incorrect.\\
Here are some examples:\\
---\\
\\
Question: To locate a choker not located in a jewelry box or boutique where would you go? Answer Choices: (a) jewelry store (b) neck (c) jewlery box (d) jewelry box (e) boutique\\
Answer: If you want to locate a choker that is not in a jewelry box or boutique, you would most likely go to your neck (b) since a choker is a type of necklace that is worn around the neck. So the answer is (b).\\
Verdict: The question asks where you would find a choker if it's not located in a jewelry box or boutique. The given answer suggests that the choker would be found on your neck, which is a logical place for a choker when it is being worn.
However, the question seems to be seeking a location where one might find a choker for purchase or retrieval other than a jewelry box or boutique. The options provided are (a) jewelry store, (b) neck, (c) jewelry box, (d) jewelry box, and (e) boutique.\\
Considering the context, option (a) jewelry store is the most appropriate answer. A jewelry store is a common place to find chokers for purchase or display, apart from a jewelry box or boutique. The given answer assumes the choker is being worn, which is not necessarily implied by the question.
So the verdict is: [[wrong]]\\
\\
---\\
......\\
---\\
\\
Question: Stanley had a dream that was very vivid and scary. He had trouble telling it from what? Answer Choices: (a) reality (b) imagination (c) dreamworker (d) nightmare (e) awake\\
Answer: The answer should be something that Stanley had trouble distinguishing his dream from. In this case, the answer is (a) reality. Stanley had trouble telling his vivid and scary dream from reality. So the answer is (a).\\
Verdict: The question asks what Stanley had trouble distinguishing his vivid and scary dream from. The given answer states that the correct choice is (a) reality, indicating that Stanley had difficulty telling his dream apart from real life. This interpretation is consistent with the typical use of the phrase "had trouble telling it from" in the context of dreams. It suggests that the dream felt so real to Stanley that he struggled to differentiate it from actual events or experiences.
So the verdict is: [[correct]]\\
\\
---\\
\\
Please consider the example provided and think it step by step.\\
Question: \{question\}\\
Answer: \{response\}\\
Verdict:\\
\bottomrule
\end{tabular}
}
\caption{Few-shot Prompt (4-shot) of CSQA for Critique}
\end{table*}
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{\textwidth}}
\toprule
Review the above answer and determine whether it’s correct. If wrong, find the problems with it.\\
Finally, conclude with either '[[correct]]' if the above answer is correct or '[[wrong]]' if it is incorrect.\\
Here are some examples:\\
---\\
\\
Question: Based on when the project was being worked on, when did the Manhattan project begin and end?\\
Answer: The Manhattan Project began in 1939 and ended in 1946. It was a research and development project during World War II that produced the first nuclear weapons. So the answer is: Began 1939, end 1946\\
Verdict: The Manhattan Project actually began in 1942, not 1939, and was completed in 1946. It was indeed a research and development project during World War II that led to the creation of the first nuclear weapons. The incorrect start date in the answer makes it inaccurate. So the verdict is: [[wrong]]\\
\\
---\\
\\
Question: Who helped lewis and clark on their journey?\\
Answer: Lewis and Clark were helped on their journey by the Corps of Discovery, which included members like Sacagawea, who served as an interpreter and guide. So the answer is: Sacagawea\\
Verdict: The answer to the question ""Who helped Lewis and Clark on their journey?"" is correct. Lewis and Clark were assisted by the Corps of Discovery, which included Sacagawea, an important member who served as an interpreter and guide. Therefore, the answer identifying Sacagawea as a key helper is accurate. So the verdict is: [[correct]]\\
\\
---\\
\\
Question: Who does the voice of cortana in halo video games?\\
Answer: The voice of Cortana in the Halo video games is provided by actress Jen Taylor. So the answer is: Jen Taylor\\
Verdict: The answer provided for the voice of Cortana in the Halo video games is correct. Jen Taylor is indeed the actress who voices Cortana in the series. So the verdict is: [[correct]]\\
\\
---\\
\\
Question: Who is lin's father in legend of korra?\\
Answer: In the animated series ""The Legend of Korra,"" Lin Beifong's father is Toph Beifong, who is a prominent character in the Avatar universe and one of the original members of Team Avatar from the preceding series, ""Avatar: The Last Airbender."" So the answer is: Toph Beifong\\
Verdict: In ""The Legend of Korra,"" Lin Beifong's father is not Toph Beifong. Toph Beifong is Lin's mother. Lin's father is revealed to be a man named Kanto. This information is disclosed in season 4 of the series, making the original answer incorrect. So the verdict is: [[wrong]]\\
\\
---\\
\\
Please consider the example provided and think it step by step.\\
Question: \{question\}\\
Answer: \{response\}\\
Verdict:\\
\bottomrule
\end{tabular}
}
\caption{Few-shot Prompt (4-shot) of AmbigNQ for Critique}
\end{table*}

\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{\textwidth}}
\toprule
Review the above answer and determine whether it’s correct. If wrong, find the problems with it.\\
Finally, conclude with either '[[correct]]' if the above answer is correct or '[[wrong]]' if it is incorrect.\\
Here are some examples:\\
---\\
\\
Question: Herman likes to feed the birds in December, January and February.  He feeds them 1/2 cup in the morning and 1/2 cup in the afternoon.  How many cups of food will he need for all three months?\\
Answer: Herman feeds the birds 1/2 cup in the morning and 1/2 cup in the afternoon, so each day he uses 1/2 + 1/2 = 1 cup of food. There are 3 months in total, so he will need 3 * 1 = 3 cups of food for all three months. The answer is 3.\\
Verdict: The answer calculates Herman feeding the birds 1 cup of food per day (1/2 cup in the morning and 1/2 cup in the afternoon). However, it incorrectly multiplies this daily amount by 3, assuming there are only 3 days in three months, resulting in 3 cups of food for all three months. This is a significant error in understanding the duration of three months.\\
So the verdict is: [[wrong]]\\
\\
---\\
......\\
---\\
\\
Question: Weng earns \$12 an hour for babysitting. Yesterday, she just did 50 minutes of babysitting. How much did she earn?\\
Answer: Weng earns \$12 per hour for babysitting. Yesterday, she babysat for 50 minutes, which is equivalent to 50/60 = 5/6 of an hour. To calculate her earnings, multiply her hourly rate by the fraction of an hour she worked: $12 * 5/6 = $10. Weng earned \$10 for her 50 minutes of babysitting. The answer is 10.\\
Verdict: The given answer accurately calculates Weng's earnings for babysitting for 50 minutes. It correctly identifies that 50 minutes is 5/6 of an hour and then multiplies this fraction by her hourly rate of \$12. The calculation of \$12 * 5/6 equals \$10, which is the correct amount Weng earned for her 50 minutes of babysitting.\\
So the verdict is: [[correct]]
\\
---\\
\\
Please consider the example provided and think it step by step.\\
Question: \{question\}\\
Answer: \{response\}\\
Verdict:\\
\bottomrule
\end{tabular}
}
\caption{Few-shot Prompt (4-shot) of GSM8K for Critique}
\end{table*}
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{\textwidth}}
\toprule
Review the above answer and determine whether it’s correct. If wrong, find the problems with it.\\
Finally, conclude with either '[[correct]]' if the above answer is correct or '[[wrong]]' if it is incorrect.\\
Here are some examples:\\
---\\
......\\
---\\
\\
Table:\\
$[$TITLE$]$: Ferry fares\\
Ferry | Car | Bicycle\\
Seattle-Bremerton | \$12 | \$8\\
Mukilteu-Clinton | \$7 | \$5\\
Southport-Fort Fisher | \$5 | \$2\\
Fauntleroy-Vashon | \$15 | \$5\\
Ocracoke | \$15 | \$3\\
Question: For an economics project, Layla determined the cost of ferry rides for bicycles and cars. How much does it cost to take a bicycle on the Southport-Fort Fisher ferry?
Answer: To find the cost of taking a bicycle on the Southport-Fort Fisher ferry, you can refer to the table:\\
Southport-Fort Fisher | \$5 | \$2\\
The cost for a bicycle on the Southport-Fort Fisher ferry is \$2.\\
So, it costs \$2 to take a bicycle on this ferry.
The answer is 2.\\
Verdict:\\
Upon reviewing the provided answer:\\
The question asks for the cost of taking a bicycle on the Southport-Fort Fisher ferry.
The table provides the cost of ferry rides for both cars and bicycles.\\
The entry for the Southport-Fort Fisher ferry shows the cost for a bicycle as \$2.\\
The answer correctly identifies this value from the table and states that it costs \$2 to take a bicycle on the Southport-Fort Fisher ferry.
No calculations are needed as the information is directly available in the table.\\
The answer accurately extracts the relevant data from the table and correctly identifies the cost of taking a bicycle on the Southport-Fort Fisher ferry as \$2.\\
So the verdict is: [[correct]]\\
\\
---\\
\\
Please consider the example provided and think it step by step.\\
Question: \{question\}\\
Answer: \{response\}\\
Verdict:\\
\bottomrule
\end{tabular}
}
\caption{Few-shot Prompt (4-shot) of TabMWP for Critique}
\end{table*}

\begin{table*}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{\textwidth}}
\toprule
Review the provided answer and determine whether it’s correct. If wrong, find the problems with it.\\
Finally, conclude with either '[[correct]]' if the provided answer is correct or '[[wrong]]' if it is incorrect.\\
Here are some examples:\\
---\\
\\
Question: Say pickup a pound of green beans twice, replacing a pound with a bunch for even times and a handful for odd\\
Answer: pickup a handful of green beans pickup a bunch of green beans\\
Verdict: Let's break down the instruction:\\
The instruction is to "pick up a pound of green beans twice".\\
For even times, replace "a pound" with "a bunch".\\
For odd times, replace "a pound" with "a handful".\\
Following these instructions:\\
The first time (odd), "pick up a pound of green beans" becomes "pick up a handful of green beans".
The second time (even), "pick up a pound of green beans" becomes "pick up a bunch of green beans".
Therefore, the provided answer of "pick up a handful of green beans pick up a bunch of green beans" matches the instructions given.\\
So the verdict is: [[correct]]\\
\\
---\\
...\\
---\\
\\
Question: Say stack ten bricks three times, replacing ten with twenty for even times and five for odd times.\\
Answer: stack five bricks stack twenty bricks stack ten bricks.\\
Verdict: According to the instruction:\\
Say "stack ten bricks" three times.\\
Replace "ten" with "twenty" for even times.\\
Replace "ten" with "five" for odd times.\\
Applying these rules:\\
First time (odd): Replace "ten" with "five", resulting in "stack five bricks".\\
Second time (even): Replace "ten" with "twenty", resulting in "stack twenty bricks".\\
Third time (odd again): Replace "ten" with "five", resulting in "stack five bricks".\\
The provided answer incorrectly says "stack ten bricks" for the third time instead of replacing "ten" with "five".
So the verdict is: [[wrong]]\\
\\
---\\
\\
Please consider the example provided and think it step by step.\\
Question: \{question\}\\
Answer: \{solution\}\\
Verdict:\\
\bottomrule
\end{tabular}
}
\caption{Few-shot Prompt (4-shot) of Repeat Copy for Critique}
\end{table*}


==> text/7_impact.tex <==
\section{Impact Statements}
\textbf{Ethical Impacts} This study does not raise any ethical concerns. 

\textbf{Expected Societal Implications} 

